Modelling of IP Geolocation by use of Latency Measurements

IP Geolocation is a key enabler for many areas of application like Content Delivery Networks, targeted advertisement and law enforcement. Therefore, an increased accuracy is needed to improve service quality. Although IP Geolocation is an ongoing field of research for over one decade, it is still a challenging task, whereas good results are only achieved by the use of active latency measurements. This paper presents an novel approach to find optimized Landmarks positions which are used for active probing and introduce an improved location estimation. Since a reasonable Landmark selection is important for a highly accurate localization service, the goal is to find Landmarks close to the target with respect to the infrastructure and hop count. Current techniques provide less information about solving this problem as well as are using imprecise models. We demonstrate the usability of our approach in a real-world environment. The combination of an optimized Landmark selection and advanced modulation results in an improved accuracy of IP Geolocation.

==> scenario.tex <==
\section{Scenario and Requirements}\label{sec:scenario}
%
The need for an accurate and reliable Geolocation service is illustrated by using the following real-world scenario. A sophisticated attack on a company network is detected by a behaviour based IDS. The management of the company requires a clarification of the case. As part of a pre-forensic strategy, the physical location of the attack source should be localized. Therefor, a Geolocation service is necessary, which uses the determined IP address of the possible attacker and correlates delay pattern with the estimated distance \cite{Ziviani2003}.
%which can be triggered with the determined IP address of the possible attacker and correlated delay pattern with the estimated distance \cite{Ziviani2003}.
The extracted information are used to prove the evidence and to start further actions. Beside this, all data is recorded and stored with signatures to cope the forensic needs of law enforcement. %The deployed incident response team is now able cooperate with different authorities as well as the concerned ISP to trace back the attack and identify the responsible person.

Since the location of the aggressor is not known beforehand, a well distributed network of multiple Landmarks is required.
%Since the location of the aggressor is not known beforehand, a well distributed network of Landmarks for active latency measurements and multilateration is required.
%Since the location of the aggressor is not known beforehand, a widely distributed network of multiple Landmarks is required for active time measurements and Multilateration.
The chosen Vantage Points have to be close to the measured target with respect to the infrastructure and the hop count. As closer such a reference host is to the target, the impact of interfering influences during the active latency measurement is reduced. Because of the high-performance connection, the ideal case are Landmarks placed within the backbone network topology \cite{Wang2011}.
%\color{red}
The accuracy of latency measurements and the optimal selection of Landmarks is directly related to the precise detection of a nearby target. % which can be referenced by the measurement from a well known location.\color{black}\todo{bin mir nicht sicher, ob der satz das aussagt was gemeint ist?}
%The accuracy of latency measurements and the optimal selection of Landmarks is directly related to the precise detection of a nearby target that can be referenced by the measurement from a well known location.
%There are several public Landmark infrastructures, e.g. RIPE Atlas, which can be used for multipoint sampling. A corresponding amount must be selected. Alternatively, an own measurement infrastructure can be setup.
The amount of Landmarks needed is mainly influenced by the network load by applied multiple measurements and cost-efficiency in terms of maintaining a probing infrastructure.
Thus, a predetermined number of nodes have to be placed in the network topology %. %An example of such an optimization problem is shown in Figure \ref{fig:backboneTopology}. It presents the backbone network in Europe, where we need to find a predefined number k center nodes
with minimized maximum distance to the surrounding network topology. This optimization problem is NP-hard \cite{Gonzalez85} and is based on the classical k-center problem for clustering. 
%
%\vspace*{-0.3cm}
%\begin{figure}[hbtp]
%{
%\centering
%\includegraphics[width=8.80cm]{5.png}
%\includegraphics[width=0.48 \textwidth]{picture/interconnect.png}
%\caption{Example Internet backbone network topology in Europe \cite{Knight2011}.}
%\label{fig:backboneTopology}
%}
%\end{figure}
%\vspace*{-0.2cm}

Therefor, we introduce a novel strategy to find a predefined number of optimized positions in the top level network topology with known geographical coordinates. Moreover, a new approach of an advanced and more accurate mathematical modelling of the geographical location estimation process is described. % Based on optimized Landmark selection and positioning as well as the detailed model, latency measurements by use of Round-Trip-Times (RTT) are conducted.
%Due to ongoing malicious traffic, communication characteristic and delays are constantly examined, thus verifying the attack source IP and the corresponding location estimation.


